Parallelization is All System Identification Needs: End-to-end Vibration Diagnostics on a multi-core RISC-V edge device

The early detection of structural malfunctions requires the installation of real-time monitoring systems ensuring continuous access to the damage-sensitive information; nevertheless, it can generate bottlenecks in terms of bandwidth and storage. Deploying data reduction techniques at the edge is recognized as a proficient solution to reduce the system's network traffic. However, the most effective solutions currently employed for the purpose are based on memory and power-hungry algorithms, making their embedding on resource-constrained devices very challenging; this is the case of vibration data reduction based on System Identification models. This paper presents PARSY-VDD, a fully optimized PArallel end-to-end software framework based on SYstem identification for Vibration-based Damage Detection, as a suitable solution to perform damage detection at the edge in a time and energy-efficient manner, avoiding streaming raw data to the cloud. We evaluate the damage detection capabilities of PARSY-VDD with two benchmarks: a bridge and a wind turbine blade, showcasing the robustness of the end-to-end approach. Then, we deploy PARSY-VDD on both commercial single-core and a specific multi-core edge device. We introduce an architecture-agnostic algorithmic optimization for SysId, improving the execution by 90x and reducing the consumption by 85x compared with the state-of-the-art SysId implementation on GAP9. Results show that by utilizing the unique parallel computing capabilities of GAP9, the execution time is 751{\mu}s with the high-performance multi-core solution operating at 370MHz and 0.8V, while the energy consumption is 37{\mu}J with the low-power solution operating at 240MHz and 0.65V. Compared with other single-core implementations based on STM32 microcontrollers, the GAP9 high-performance configuration is 76x faster, while the low-power configuration is 360x more energy efficient.

==> image_texts/01_introduction.tex <==
\begin{figure}
  \centering
\includegraphics[width=1\columnwidth]{images/intro.pdf}
  \caption{IoT-based SHM systems.}
\label{fig:intro}
 % \vspace{-0.5cm}
\end{figure}

==> images/spectraImages.tex <==
%%% -------------------------- WT SPECTRA PLOTTING

\begin{figure*}[tb]
    \centering
    \begin{adjustbox}{width=\linewidth}
    \begin{tikzpicture}
    
    \begin{groupplot}[
    group style={
        group name=my plots,
        group size=2 by 1,
        ylabels at=edge left,
        vertical sep = 0pt,
        horizontal sep = 10pt},
    footnotesize,
    % height = 5cm,
    tickpos = left,
    ytick align = outside,
    xtick align = outside,
    enlarge x limits = false]

    \nextgroupplot[title={\tiny Z24}, label style={font=\tiny}, tick label style={font=\tiny}, xlabel = {Frequency [Hz]}, xmin = 2, xmax = 15, ymin = -110, ymax = -50, ylabel = {PSD [dB/$\sqrt{Hz}$]}, minor x tick num = 1, 
    legend style={at={(1,0.99)}, legend style={draw=none}, legend image post style={scale=0.3}, font = \tiny, anchor=north}, legend columns=3, legend cell align={left}]
    \addplot[black, line width = 0.6pt] table[x = f, y = arma1]{./images/Z24.txt};\label{arma1}
    \addplot[blue, line width = 0.6pt] table[x = f, y = arma2]{./images/Z24.txt};\label{arma2}
    \addplot[red, line width = 0.6pt] table[x = f, y = arma3]{./images/Z24.txt};\label{arma3}

    % \addplot[blue!30!white, line width = 0.6pt] table[x = f, y = ar1]{./images/Z24.txt};\label{ar1}
    % \addplot[red!30!white, line width = 0.6pt] table[x = f, y = ar2]{./images/Z24.txt};\label{ar2}
    % \addplot[green!30!white, line width = 0.6pt] table[x = f, y = ar3]{./images/Z24.txt};\label{ar3}
    
    \path[name path=axis2] (axis cs:0,-50) -- (axis cs:20,-50);
    \path[name path=axis1] (axis cs:0,-120) -- (axis cs:20,-120);
    \addplot [thick, color=gray, fill=gray, fill opacity=0.05] fill between [of=axis2 and axis1,soft clip={domain=3.3:4.2}];
    \addplot [thick, color=gray, fill=gray, fill opacity=0.05] fill between[of=axis2 and axis1,soft clip={domain=4.35:5.2}];
    \addplot [thick, color=gray, fill=gray, fill opacity=0.05] fill between[of=axis2 and axis1,soft clip={domain=5.5:7}];
    \addplot [thick, color=gray, fill=gray, fill opacity=0.05] fill between[of=axis2 and axis1,soft clip={domain=9:10.5}];
    \addplot [thick, color=gray, fill=gray, fill opacity=0.05] fill between[of=axis2 and axis1,soft clip={domain=11.3:13.5}];

    % f1
    \addplot[mark=mystarc, only marks] coordinates { (4, -72)};
    \draw [dashed, line width = 0.6pt] (4,-110) -- (4,-72);
    \addplot[mark=square, only marks, fill= black!55!white, draw = red!55!white, mark size = 1.5pt] coordinates { (3.81, -59)};
    \draw [dotted, line width = 0.2pt, color= red, semithick] (3.81,-110) -- (3.81,-59);
    \addplot[mark=o, only marks, fill= black!55!white, draw = blue!55!white, mark size = 1.5pt] coordinates { (3.87, -79)};
    \draw [dotted, line width = 0.2pt, color= blue, semithick] (3.87,-110) -- (3.87,-79);
    \draw [->, line width = 0.45pt, color = gray] (4,-105) -- (3.87,-105);

    % f2
    \addplot[mark=mystarc, only marks] coordinates { (5.12, -78.61)};
    \draw [dashed, line width = 0.6pt] (5.12,-110) -- (5.12,-78.61);
    \addplot[mark=square, only marks, draw = red!55!white, mark size = 1.5pt] coordinates { (4.77, -81)};
    \draw [dotted, line width = 0.2pt, color= red, semithick] (4.77,-110) -- (4.77,-81);
    \addplot[mark=o, only marks, fill= black!55!white, draw = blue!55!white, mark size = 1.5pt] coordinates { (4.57, -97.3)};
    \draw [dotted, line width = 0.2pt, color= blue, semithick] (4.57,-110) -- (4.57,-97.3);
    \draw [->, line width = 0.45pt, color = gray] (5.12,-105) -- (4.57,-105);

    % f3
    \addplot[mark=mystarc, only marks] coordinates { (6.32, -75)};
    \draw [dashed, line width = 0.6pt] (6.32,-110) -- (6.32,-75);
    \addplot[mark=square, only marks, fill= black!55!white, draw = red!55!white, mark size = 1.5pt] coordinates { (6.44, -88)};
    \draw [dotted, line width = 0.2pt, color= red, semithick] (6.44,-110) -- (6.44,-88);
    \addplot[mark=o, only marks, fill= black!55!white, draw = blue!55!white, mark size = 1.5pt] coordinates { (6.02, -88)};
    \draw [dotted, line width = 0.2pt, color= blue, semithick] (6.02,-110) -- (6.02,-88);
    \draw [->, line width = 0.45pt, color = gray] (6.32,-105) -- (6.02,-105);

    % f4
    \addplot[mark=mystarc, only marks] coordinates { (10.01, -70.95)};
    \draw [dashed, line width = 0.6pt] (10.01,-110) -- (10,-70.95);
    \addplot[mark=square, only marks, fill= black!55!white, draw = blue!55!white, mark size = 1.5pt] coordinates { (9.81, -91)};
    \draw [dotted, line width = 0.2pt, color= blue, semithick] (9.81,-110) -- (9.81,-91);
    \addplot[mark=o, only marks, fill= black!55!white, draw = red!55!white, mark size = 1.5pt] coordinates { (9.69, -81)};
    \draw [dotted, line width = 0.2pt, color= red, semithick] (9.69,-110) -- (9.69,-81);
    \draw [->, line width = 0.45pt, color = gray] (10.01,-105) -- (9.69,-105);

    % f5
    \addplot[mark=mystarc, only marks] coordinates { (12.82, -69.99)};
    \draw [dashed, line width = 0.6pt] (12.82,-110) -- (12.82,-69.99);
    \addplot[mark=square, only marks, fill= black!55!white, draw = blue!55!white, mark size = 1.5pt] coordinates { (12.24, -86)};
    \draw [dotted, line width = 0.2pt, color= blue, semithick] (12.24,-110) -- (12.24,-86);
    \addplot[mark=o, only marks, fill= black!55!white, draw = red!55!white, mark size = 1.5pt] coordinates { (11.73, -83)};
    \draw [dotted, line width = 0.2pt, color= red, semithick] (11.73,-110) -- (11.73,-83);
    \draw [->, line width = 0.45pt, color = gray] (12.82,-105) -- (11.73,-105);
    
    
    % \draw[->, line width=1pt] (504,-150) -- (455,-150);
    
    
    \addlegendentry{\tiny Healthy}
    \addlegendentry{\tiny Mid dam}
    \addlegendentry{\tiny Sev dam}
    

    \nextgroupplot[title={\tiny Wind turbine}, label style={font=\tiny}, tick label style={font=\tiny}, xlabel = {Frequency [Hz]}, xmin = 80, xmax = 350, ymin = -40, ymax = 10, ylabel = {}, yticklabels = {}, minor x tick num = 2 ]
    \addplot[black, line width = 0.6pt] table[x = f, y = arma1, col sep=comma]{./images/WT.txt};
    \addplot[blue, line width = 0.6pt] table[x = f, y = ar2, col sep=comma]{./images/WT.txt};
    \addplot[red, line width = 0.6pt] table[x = f, y = arma3, col sep=comma]{./images/WT.txt};

    % \addplot[blue!30!white, line width = 0.6pt] table[x = f, y = ar1]{./images/WT.txt};
    % \addplot[red!30!white, line width = 0.6pt] table[x = f, y = ar2]{./images/WT.txt};
    % \addplot[green!30!white, line width = 0.6pt] table[x = f, y = ar3]{./images/WT.txt};

    \path[name path=axis2] (axis cs:60,10) -- (axis cs:350,10);
    \path[name path=axis1] (axis cs:60,-40) -- (axis cs:350,-40);
 
    \addplot [thick, color=gray, fill=gray, fill opacity=0.05] fill between[of=axis2 and axis1,soft clip={domain=110:124}];
    \addplot [thick, color=gray, fill=gray, fill opacity=0.05] fill between[of=axis2 and axis1,soft clip={domain=128:147}];
    \addplot [thick, color=gray, fill=gray, fill opacity=0.05] fill between[of=axis2 and axis1,soft clip={domain=190:225}];
    \addplot [thick, color=gray, fill=gray, fill opacity=0.05] fill between[of=axis2 and axis1,soft clip={domain=275:285}];
    \addplot [thick, color=gray, fill=gray, fill opacity=0.05] fill between[of=axis2 and axis1,soft clip={domain=290:310}];

    % f1
    \addplot[mark=mystarc, only marks] coordinates { (123, -6.54)}; 
    \draw [dashed, line width = 0.6pt] (123,-40) -- (123,-6.54);
    \addplot[mark=square, only marks, draw = blue!55!white, mark size = 1.5pt] coordinates { (116.8, -1.28)};
    \draw [dotted, line width = 0.2pt, color= blue, semithick] (116.8,-40) -- (116.8,-1.28);
    \addplot[mark = o, only marks, fill= black!55!white, draw = red!55!white, mark size = 1.5pt] coordinates { (113, -3.22)};
    \draw [dotted, line width = 0.2pt, color= red, semithick] (113,-40) -- (113,-3.22);
    \draw [->, line width = 0.45pt, color = gray] (123,-35) -- (113,-35);

    % f2
    \addplot[mark=mystarc, only marks] coordinates { (141, -7.7)}; 
    \draw [dashed, line width = 0.6pt] (141,-40) -- (141,-7.7);
    \addplot[mark=square, only marks, draw = blue!55!white, mark size = 1.5pt] coordinates { (136.5, -4.1)};
    \draw [dotted, line width = 0.2pt, color= blue, semithick] (136.5,-40) -- (136.5,-4.1);
    \addplot[mark = o, only marks, fill= black!55!white, draw = red!55!white, mark size = 1.5pt] coordinates { (128, -4.76)};
    \draw [dotted, line width = 0.2pt, color= red, semithick] (128,-40) -- (128,-4.76);
    \draw [->, line width = 0.45pt, color = gray] (141,-35) -- (128,-35);

    % f3
    \addplot[mark=mystarc, only marks] coordinates { (215, 0.9)}; 
    \draw [dashed, line width = 0.6pt] (215,-40) -- (215,0.9);
    \addplot[mark=square, only marks, draw = blue!55!white, mark size = 1.5pt] coordinates { (206.6, 0.51)};
    \draw [dotted, line width = 0.2pt, color= blue, semithick] (206.6,-40) -- (206.6,0.51);
    \addplot[mark=o, only marks, fill= black!55!white, draw = red!55!white, mark size = 1.5pt] coordinates { (195, -2.68)};
    \draw [dotted, line width = 0.2pt, color= red, semithick] (195,-40) -- (195,-2.68);
    \draw [->, line width = 0.45pt, color = gray] (215,-35) -- (195,-35);

    % f4
    \addplot[mark=mystarc, only marks] coordinates { (286.5, -9.9)}; 
    \draw [dashed, line width = 0.6pt] (286.5,-40) -- (286.5,-9.9);
    % \addplot[mark=square, only marks, draw = blue!55!white, mark size = 1.5pt] coordinates { (285.81, -12.29)};
    \addplot[mark=o, only marks, fill= black!55!white, draw = red!55!white, mark size = 1.5pt] coordinates { (280.54, -4.08)};
    \draw [dotted, line width = 0.2pt, color= red, semithick] (280.54,-40) -- (280.54,-4.08);
    \draw [->, line width = 0.45pt, color = gray] (286.5,-35) -- (280.54,-35);

    % f5
    \addplot[mark=mystarc, only marks] coordinates { (304.98, -1.84)}; 
    \draw [dashed, line width = 0.6pt] (304.98,-40) -- (304.98,-1.84);
    \addplot[mark=square, only marks, draw = blue!55!white, mark size = 1.5pt] coordinates { (298.3, -0.03)};
    \draw [dotted, line width = 0.2pt, color= blue, semithick] (298.3,-40) -- (298.3,-0.03);
    \addplot[mark=o, only marks, fill= black!55!white, draw = red!55!white, mark size = 1.5pt] coordinates { (293.45, 1.85)};
    \draw [dotted, line width = 0.2pt, color= red, semithick] (293.45,-40) -- (293.45,1.85);

    
    \draw [->, line width = 0.45pt, color = gray] (304.98,-35) -- (293.45,-35);
    
    \end{groupplot}
    \end{tikzpicture}
 \end{adjustbox}   
    \caption{Spectra for the Z24 bridge use case (left) and wind turbine blade (right) obtained by the PARSY-VDD end-to-end application deployed at the extreme edge. In both cases, one signal in healthy conditions (black profiles) and in two differently damaged conditions (blue and red for mid and highly severe, respectively) are considered.}
    \label{fig:spectra}
   
\end{figure*}

==> tables/isd_table.tex <==
\begin{table}[tb]
  \centering
  \caption{ISD values for different configurations of the deployment. On the top part, a sweep over the number of cores, while on the below part, varying $N$ and $N_p$.}
  \label{tab:isd_old}
  {
  \begin{tabular}{c|cc}
    \hline \hline
        \# cores ($N = 25\times N_p$, $N_p = 8)$ &  \textbf{AR} & \textbf{ARMA}\\ \hline
        1 & 8.33E-07 & 0.61E-03 \\  
        2 & 6.02E-07 & 0.27E-03 \\  
        4 & 1.02E-06 & 0.29E-03 \\  
        8 & 8.77E-07 & 0.13E-03 \\ 
        \hline
        \hline
        $N \times N_p$ (8 cores) &  & \\  \hline
        $[400 \times 8]$ & 8.77E-07 & 0.13E-03 \\  
        $[480 \times 16]$ & 1.24E-06 & 0.22E-04 \\  
        $[2520 \times 56]$ & 1.45E-06 & 9.14E-05 \\ 
        \hline
        \hline
  \end{tabular}
  }
\end{table}






















==> text/01_b_motivations.tex <==
Parallel programming includes a set of techniques adopted across multiple computing domains to divide computational tasks into smaller sub-tasks that can run simultaneously. In embedded systems characterized by demanding workloads coupled with stringent power budgets, parallel programming plays a crucial role in reducing energy consumption.
Specifically, \emph{parallel near-threshold computing} is an architectural paradigm that leverages parallel processing and near-threshold voltage operation to achieve these goals.
Operating transistors at near-threshold voltages reduces the energy consumed per operation, while parallel processing allows for higher computational throughput; combining these techniques can drastically improve energy efficiency at the system level.

The Parallel Ultra-Low-Power (PULP) platform is a microcontroller-class architecture including a programmable accelerator cluster that leverages parallel near-threshold computing.
In this platform, parallel processing on the cluster allows for higher computational throughput without significantly increasing overall power consumption; at the same time, reducing the overall computation time implies a reduction of energy consumption.
Moreover, a dedicated hardware block (\emph{event unit}) handles synchronization primitives and puts unused cores in a low-power idle state; this feature further reduces the system-level power consumption when the workload is not balanced, a common condition in signal processing algorithms.
We performed an experimental assessment of our solution on GAP9, a commercial embodiment of the PULP platform described in ~\secref{subsec_gap9_theory}.

==> text/02_a_qr_decomposition.tex <==


% One of the core computing functions at the basis of SysId, QR decomposition is a linear algebra operation particularly useful to solve linear least squares systems and eigenvalue problems. Therefore, 
The implementation of QR on low-end devices requires particular attention and has attracted interest from many researchers in the last decades since it is particularly useful in solving linear least squares systems and eigenvalue problems.

In recent studies, Le \textit{et al.}~\cite{le2023block} proposed a new QR decomposition approach that recursively applies the block variant of the Householder method in larger blocks, exceeding a single column in size, which aims to ensure both stability and computational efficiency. Buttari \textit{et al.}~\cite{buttari2009class} employed LAPACK to present QR factorization algorithms. In their approach, operations are represented as a sequence of small tasks that can be dynamically scheduled for execution. The resulting out-of-order task execution increases the parallelism, local data reuse, and hiding the latency of memory accesses, resulting in high performance on multi-core architectures. 
In another study, Ida \textit{et al.}~\cite{ida2019qr} leveraged Intel MKL to present a parallel QR factorization using a block low-rank (BLR-) matrix representation, which results in faster execution on multi-core platforms. \cite{terao2020lu}~proposed a method for thin QR decomposition using LU-Cholesky QR algorithms. They utilized LU factors of a given matrix as preconditioning before applying Cholesky decomposition, which led to increased speed-up in shared and distributed memory systems without compromising orthogonality.

Considering GPU platforms as a target, Kerr et al.~\cite{Kerr2009QRDO} explore architectural features and propose a strategy for high-performance QR decomposition using cuBLAS. Ohshima et al. ~\cite{ohshima2022qr} extend the concept of BLR-QR factorization to GPUs, inspired by the approach in~\cite{ida2019qr}, aiming to reduce memory usage while enhancing acceleration with cuBLAS and cuSOLVER.
Merchant et al. ~\cite{Merchant2018}~focus on efficient Householder implementation as part of algorithm-architecture co-design, incorporating LAPACK, PLASMA, and MAGMA libraries. This approach aims to maximize throughput and minimize latency on single-core, multi-core, and GPU platforms by tailoring the algorithm to specific hardware. 

Most of the techniques proposed for HPC systems and GPUs described in the previous paragraphs are unsuitable for the embedded domain. The matrix size for embedded applications is typically smaller, making block approaches inconvenient. Moreover, the architecture of PULP platforms highly differs from GPUs, requiring ad hoc approaches for code optimization.

In the FPGA domain, researchers have concentrated on creating QR decomposition accelerators exploiting the spatial parallelism largely available on reconfigurable devices. Muñoz \textit{et al.}~\cite{munoz2015high} and Wang \textit{et al.}.~\cite{wang2009truly} have contributed designs utilizing Givens rotations within 2-D systolic arrays featuring pipelined CORDIC-based processing elements. Expanding this FPGA-focused field, Langhammer \textit{et al.}~\cite{Langhammer2018} introduced a unique approach. They adapted the loop structures of the Gram-Schmidt algorithm and proposed a novel QRD algorithm. This algorithm was then mapped onto parallel structures with inter-vector connectivity, which led to an increasing performance ratio for medium and large-size matrices.
In this work, we focus on optimizing a set of QR algorithms for general-purpose parallel platforms for IoT computing. Our target is a programmable accelerator able to execute diverse workloads, so our optimization efforts are more focused on the software side, and we do not consider the optimization enabled by reconfigurable logic.

Focusing on software contributions, Eigen is a C++ template library including linear algebra algorithms. It supports integer and floating-point operations, efficiently using the most widespread Single Instruction Multiple Data (SIMD) instruction sets~\cite{eigenweb}.
In the IoT and embedded domains, ARM contributes with ARM CMSIS (Cortex Microcontroller Software Interface Standard), designed for Cortex-M microcontrollers. By providing a unified interface for core functions and hardware features, this library simplifies embedded software development~\cite{ARM-CMSIS}.
Zonzini et al.~\cite{Zonzini2022} introduced an adaptation of the sequential tall-skinny QR decomposition (eS-TSQR), originally designed for dense linear algebra. This tailored approach efficiently addresses memory and computational challenges, making it well-suited for resource-constrained embedded devices. 
Open-source libraries such as PULP-DSP~\cite{pulpdsp} and TransLib~\cite{Mirsalari2023} combine parallel processing and reduced-precision arithmetic, saving memory and execution time. These optimizations consider diverse RISC-V ISA extensions and are highly beneficial for PULP platforms.

In this work, we expand the capabilities of the PULP-DSP library by designing fine-tuned variants of the QR decomposition. 
Analyzing the current research, no existing library in the embedded domain incorporates all three variants. Furthermore, our optimization efforts are tailored to align with the specific demands and constraints of IoT devices and designed for one order of magnitude more efficient architectures than the current state-of-the-art ARM Cortex architectures.

==> text/02_b_System_identification.tex <==



Implementing SysId algorithms involves computational and memory-intensive operations, which justify the lack of experimental evidence for embedding SysId on tiny devices near the sensors. 
%
The proof is that, so far, only a few research works have been disseminated in the literature.
%
An embryonic trial was made by Hann \textit{et al.} in ~\cite{hann2009real} by providing a C language script of a SysId library, while no deployment on edge devices was demonstrated.     
%
The first relevant example is provided in~\cite{kim2012autonomous} which showcased SysId on the Narada sensor platform, i.e., one of the pristine and widely employed acceleration sensors for SHM based on the Atmel ATmega128 MCU operating at \SI{8}{MHz} clock frequency and maximum storage capabilities of \SI{128}{kBytes} of RAM and flash. However, the system hardware/software constraints imposed the adoption of correlation-based SysId variants, hampering its effective exploitation as an efficient data reduction method. 
%


Field Programmable Gate Arrays (FPGA) are a feasible target for real-time deployment of SysId~\cite{atencia2007fpga, biradar2015fpga, boumeridja2005fpga}. Nevertheless, deploying FPGA-based systems at the edge is not intuitive due to their energy-demanding nature, {as they are mostly grid-based systems and consume an order of magnitude more energy than the commercially available MCUs at the edge.}
%





%
More recently, authors in \cite{zonzini2022system} achieved successful deployment on a general-purpose prototype sensor equipped with an STM32L5 based on an Arm\textregistered Cortex\textregistered-M33 MCU; however, this solution is affected by long execution time (greater than \SI{120}{s} in the most cumbersome scenario) due to the sequential nature of the computational workflow forced by the single-core architecture of the computing processor. 
%
Notably, \cite{moallemi2023speeding} overcomes most of the issues above by proposing a parallelized version of the linear algebra operators at the core of SysId. Nevertheless, they merely provide a solution for the specific 8-core device, while we present a configurable implementation of SysId suitable for all MCU edge devices. 
% 
% Moreover, not only QR decomposition but also other parts of the SysId are parallelized, which has not been done in~\cite{moallemi2023speeding}.  
%
% Further, by fitting all the computations in the \lone memory combined with parallized and optimized implementation, we decrease latency by $\approx$ \qty{27}{\times} from \qty{68}{\milli \second} to \qty{2.5}{\milli \second}. 
% 
%
% Finally, we compare several processors and resource-constrained devices, showcasing the difference between conventional single-core edge devices and emerging multi-core ones.  
% Eventually, this evidences the lack of on-sensor SysId implementations compatible with continuous and real-time diagnostic functionalities.
%
